Energy Optimal Transmission Scheduling in Wireless Sensor Networks

One of the main issues in the design of sensor networks is energy efficient communication of time-critical data. Energy wastage can be caused by failed packet transmission attempts at each node due to channel dynamics and interference. Therefore transmission control techniques that are unaware of the channel dynamics can lead to suboptimal channel use patterns. In this paper we propose a transmission controller that utilizes different "grades" of channel side information to schedule packet transmissions in an optimal way, while meeting a deadline constraint for all packets waiting in the transmission queue. The wireless channel is modeled as a finite-state Markov channel. We are specifically interested in the case where the transmitter has low-grade channel side information that can be obtained based solely on the ACK/NAK sequence for the previous transmissions. Our scheduler is readily implementable and it is based on the dynamic programming solution to the finite-horizon transmission control problem. We also calculate the information theoretic capacity of the finite state Markov channel with feedback containing different grades of channel side information including that, obtained through the ACK/NAK sequence. We illustrate that our scheduler achieves a given throughput at a power level that is fairly close to the fundamental limit achievable over the channel.

==> concl.tex <==
\section{Conclusions}\label{sec:concl}
\vspace{-0.1in}
We introduced a channel aware transmission scheduler to optimize energy efficiency in sensor networks. Our transmission scheduler meets the deadline constraint for all packets waiting in the transmission queue while optimizing the total energy spent on transmission. To do this, we used finite-horizon DP and utilized different types of CSI in the optimization process. 
%This scheduler can be employed in existing networks since it does not require additional hardware and we provide a simple implementation as an illustration. 
We also derived the capacity-cost function of a FSMC with different types of CSI at the controller. 
%For that purpose, we calculated the capacity of a FSMC with ACK/NAK feedback. To our knowledge this was an open problem. 
The capacity-cost function can be used as a bound for the performance of the transmission schedulers.
We showed that the performance achieved by a DP-based scheduler is close to the fundamental limits for a wide range of channel parameters. Indeed, for some cases, the ACK/NAK scheduler achieves performance that is within 80\% of the theoretical bound. Comparisons between the performance of different grades of CSI show that the difference between performance of causal perfect CSI and ACK/NAK schemes for a wide range of channel parameters is not significant. On the other hand, blind transmission scheme in which the ACK/NAK feedback is not exploited to estimate the channel state incurs a significant power penalty. In addition, the maximum power penalty incurred by ACK/NAK feedback based schemes provide insights into the fundamental value of using ACK/NAK information while scheduling transmissions. For instance, in one case, the maximum power penalty of not using any kind of feedback is 4.5 dB. The use of ACK/NAK information, which is available to the transmitter in most wireless link layer protocols without extra effort, can reduce this power penalty to less than 1 dB. 

%We derived the capacity-cost function for finite state Markov channels with different feedback information. In this case channel inputs have discrete power levels and a long term average power constraint. To the best of our knowledge, the capacity-cost function for such channels have not been derived previously. 
%Of special interest is the finite state Markov channel with ACK/NAK feedback. 
%The capacity-cost function found here can be used as a bound for the throughput performance of ON-OFF schedulers. In addition, the maximum power penalty incurred by ACK/NAK feedback based schemes provide insights into the fundamental value of using ACK/NAK information while scheduling transmissions. For instance, in bursty channels, the maximum power penalty of not using any kind of feedback is 7 dB. The use of ACK/NAK information, which is freely available to the transmitter, can reduce this power penalty to less than 1 dB. On the other hand, in reliable channels (average probability of error $< 0.1$) the advantage of using ACK/NAK feedback over no feedback is almost negligible.
%We also showed that in many cases, channel probing can be wasteful in terms of energy efficiency, even when the probing cost is no more than 7\% of the cost of transmitting a full data packet.




==> intro.tex <==
\section{Introduction}\label{sec:intro}
\vspace{-0.1in}
%One way to tackle this problem is to adapt transmission parameters (e.g.~Power, Codes) to the channel and data states. For instance, the scheduler should slow down the transmission rate when the probability of a packet loss is high. 
Energy efficient communication is one of the key concerns in the design of
wireless sensor networks. Without any effort for adapting to the variability
in the channel, the system resources are consumed inefficiently. For instance,
if bad channel conditions are not anticipated, a high fraction of the node
energy can be consumed by multiple retransmissions per correctly decoded
packet. To avoid such inefficiencies, sensor nodes use transmission schedulers.
The objective of an energy-efficient transmission scheduler is to reliably communicate data using minimal amount of energy, while meeting deadline
and/or throughput constraints. Design of efficient transmission schedulers is
challenging - especially in sensor networks - due to limited computational
resources and the lack of perfect channel side information (CSI) at the
transmitter.
Transmitters used in sensor networks often do not have access to advanced modulation techniques, which rules out the use of sophisticated adaptive transmission schemes.
% Transmitter design limitations in sensor networks also do not allow sophisticated adaptive transmission schemes. 

Consequently we focus our attention on transmission
schemes that do not require a high computational power. 
%The channel model that we consider for this problem is a finite-state Markov erasure channel (FSMEC). A FSMC is a channel model which, during each symbol duration, is in one of a finite number of states with Markov transition between these states. A FSMEC is a special case of FSMC, where each state has an erasure channel (EC)~\cite{CoverBook} associated with it. 
We propose a transmission scheduler that utilizes different
``grades'' of CSI on the state of a FSMC to schedule
packet transmissions in order to meet a deadline constraint for the packets
waiting in the transmission queue. We are specifically interested
in the highly imperfect CSI that can be obtained based solely on the ACK/NAK
sequence for the past transmissions. 
%Note that, this level of information is freely available at
%the link layer in almost all wireless networks. Therefore it does not require
%an extra effort (such as sending special non-information carrying
%physical-layer pilot symbols over the channel) to obtain.  
Note that, this level of information is available at the link layer in almost all wireless networks without any extra effort (such as sending special non-information carrying physical-layer pilot symbols over the channel). Our transmitter has
a single transmit power level and the coding and modulation schemes are fixed.
In every transmission opportunity, the transmitter can choose to attempt the
packet transmission or defer it.
%based on the buffer state and some estimate of the channel state at the time.

Our scheduler is based on the dynamic programming (DP)
solution to a finite-horizon transmission control problem. We show how a simple version of it can be implemented in sensor nodes.
%We show how a simple version of it can be implemented in sensor nodes, without sacrificing much in performance. 
We also calculate the capacity-cost function of the FSMC with
feedback containing different grades of CSI. To our best knowledge, the capacity of channels with a feedback that
is a random function of the channel state (e.g., ACK/NAK) has not been
addressed before. We finally evaluate the performance of our scheduler and
illustrate that it achieves a given throughput at a power level that is fairly
close to the fundamental limit achievable over the channel.

In the transmission scheduling problem, the parameter we minimize is the
number of transmission attempts, subject to a deadline constraint for the
packets in the queue. One can realize that, with the limitation of binary
power control (transmit or do not transmit), the number of transmissions is
proportional to the energy consumed per correctly decoded packet and the deadline
constraint can be translated into a throughput constraint at every point in
time\footnote{For instance if the buffer contains 5 packets with a deadline
constraint of 1 sec, then the scheduler has to guarantee a minimum of 5
packets/sec for the next second}. Hence the problem can be viewed as minimizing
the energy per packet subject to a throughput constraint. 

%Transmission strategies based on channel estimation in FSMCs have been considered in various works. In~\cite{Zorzi97TComp,Chiasserini03TVT}, authors consider different opportunistic transmission schemes which use a two-state Markov channel similar to the one used in this work. These schemes detect a bad channel state upon receipt of a NAK. They respond to a bad channel condition by reducing the transmission rate while probing the channel periodically. The transmitter returns to normal operation when the channel improves. In contrast, we develop an algorithm that uses the ACK/NAK information, which is freely available, in conjunction with a DP-based algorithm to optimally schedule the transmission. 
%The computational overhead of our approach is also minimal and our algorithm requires two table look-ups and three basic arithmetic operations\ignore{ as we will see in Section~\ref{sec:algorithm}}. 

%In~\cite{Uysal02TNet,Zafer07ITA}, the authors have considered a problem setup similar to ours and find a stochastic rate control policy for their problem. In these works, the authors have the freedom to vary packet transmission times and power levels which require sophisticated and expensive transmitter design. %In our case however, the controller does not have access to such rate control schemes and has only discrete power levels. 
%Our solution methodology is also different as it uses the available channel state information in the {\it dynamic programming algorithm} to schedule transmissions accordingly. 

%In \cite{Chiasserini03TVT}, the transmitter switches to a greedy mode (immediate retransmission on error) when the buffer level exceeds a certain threshold to ensure that the quality of service (QoS) requirement is being met. In contrast, our algorithm is able to dynamically adapt to the QoS deadline requirement by considering the queue state in addition to the channel state to schedule transmissions.

%If the transmitter had a perfect estimate of the channel state at every point
%in time, designing a transmission scheduler would be straightforward. However,
%in almost all wireless networks, perfect CSI is not available at the
%transmitter. It is imperative to build transmission schedulers that are capable
%of exploiting imperfect CSI. Our scheduler will be based on imperfect CSI,
%obtained through the packet-level ACK/NAK sequence. 

Transmission strategies based on channel estimation in FSMCs have been considered by Zorzi and Rao~\cite{Zorzi97TComp} as well as Chiasserini and Meo~\cite{Chiasserini03TVT}. These papers assume a two-state Markov chain and detect the bad channel state upon receipt of a NAK. Both schemes reduce the transmission rate and constantly probe the channel as a response. In~\cite{Chiasserini03TVT}, the transmitter switches to a greedy transmission mode when the buffer level exceeds a certain threshold, regardless of the channel state. Our scheme is based on a dynamic program, which takes the queue and the estimated channel states jointly into account to schedule packet transmissions in an optimal manner.
%We use a DP approach to solve different versions of this problem. We also discuss implementation details of the
%solution and provide an implementable approximate version of our DP-based
%scheduler for sensor networks.
Johnston and Krishnamurthy~\cite{Johnston06TWC} give an algorithm that minimizes the transmission energy and latency while transmitting over a fading channel by formulating the problem as a partially observed Markov decision process (POMDP) search problem. However, their threshold-based policy result is optimal for a 2-state channel only. In addition, the channel model is assumed to have a unity packet loss probability in one state. This may not seem like a fundamental difference, but in such a scenario, an ACK implies a ``good'' state. The corresponding time dependence is finite and the associated solution can exploit it. Our results are valid for a general FSMC. 

Uysal, et.~al.,~\cite{Uysal02TNet} and Zafer, et.~al.,~\cite{Zafer07ITA} have considered rate control policies for transmission scheduling similar to ours. However,~\cite{Uysal02TNet} uses a static channel model for deriving the control policy. On the other hand,~\cite{Zafer07ITA} considers a Markov channel, but assumes knowledge of the channel state prior to transmission. 
In our model, this information is not available to the controller. 
Haleem, et.~al.,~\cite{Haleem05JSAC} use ACK/NAK feedback in a learning automata algorithm to schedule transmissions. This method is shown to converge to the optimal throughput in stationary channels. Ho, et.~al.,~\cite{Ho06VTC} give a sub-optimal rate adaptation scheme to maximize throughput that uses ACK/NAK feedback. Karmokar, et.~al.,~\cite{Karmokar06TWC2} pose the problem of rate adaptation in Type-I Hybrid ARQ systems as a POMDP and provide some heuristic solutions. The authors develop this idea further and propose a linear programming approach to solve the POMDP problem~\cite{Djonin08TVT,Karmokar08TComm}.

%Our solution methodology is also different as it uses the available channel state information in the {\it dynamic programming algorithm} to schedule transmissions. 

In the second part of the paper, we study fundamental limitations of FSMCs with feedback containing perfect and imperfect CSI.
We will use tools from information theory to derive the capacity results for power constrained channels. Capacity of channels with CSI is a well studied topic. Goldsmith and Varaiya~\cite{Goldsmith97TIT} gave the Shannon capacity of such channels with instantaneous CSI at the transmitter and receiver. In this case, CSI implies accurate knowledge of the instantaneous state of the Markov channel. The optimal power adaptation for such a channel model implies ``water-filling'' in time, which is analogous to the water-filling result in frequency in a frequency-selective channel~\cite{CoverBook}. Viswanathan~\cite{Viswanathan99TIT} extended these results for delayed perfect CSI at the transmitter. Y\"uksel and Tatikonda derived the capacity of a FSMC with imperfect deterministic feedback~\cite{Yuksel07ISIT}. Imperfect deterministic feedback implies that the transmitter has inaccurate (quantized) information about the channel state. The quantizer used is a deterministic function of the channel state. Although these results are useful for a wide variety of capacity calculations, they can not be applied directly to channels with discrete power levels and a long term average power constraint on the input symbols. This is due to the fact that the transmitter might have to defer transmission in order to meet the power constraints.
%However in their work, they consider deterministic quantized feedback. 

To incorporate skipped transmission attempts in the classical
capacity results, we introduce a new discrete channel, which we call
{\em{channel with vacation}}. We associate a channel with vacation to each
state of the FSMC, and calculate the capacity-cost function
for this special Markov channel. The general problem of finding the capacity
of a feedback channel with memory has been notoriously difficult in
information theory; and the problem of feedback capacity containing a CSI,
which is a random function of the channel state has not been addressed before. We use this kind of a feedback in our channel model because the probability of a transmission success is channel state dependent, which implies that the feedback is a random function of the channel state. We generalize~\cite{Yuksel07ISIT} and combine it with~\cite{Viswanathan99TIT} and~\cite{Verdu90TIT} in order to calculate the capacity-cost function of our channel with feedback.
We compare this capacity-cost function with the performance achieved by our scheduler and observe that for a given throughput requirement, the power expended by our scheme is close to the theoretical limit of the system.
%We calculate the capacity of the feedback channel with ACK/NAK feedback and illustrate that the DP based scheme achieves a given throughput at a power level that is fairly close to the fundamental limit achievable.

%authors consider different opportunistic transmission schemes which use a two-state Markov channel similar to the one used in this work.\ignore{The channel state is determined by automatic repeat request (ARQ) level information.} These schemes detect a bad channel state upon receipt of a NAK. However, they respond to a bad channel condition by reducing the transmission rate while probing the channel periodically. The transmitter returns to normal operation when the channel improves. In contrast, we develop an algorithm that uses ACK/NAK information, which is freely available, in conjunction with a DP-based algorithm to optimally schedule packet transmissions. 
%The computational overhead of our approach is also minimal and our algorithm requires two table look-ups and three basic arithmetic operations\ignore{ as we will see in Section~\ref{sec:algorithm}}. 
%the incoming traffic flow rate and thus setting an optimal pushback period that supports this throughput. 


%In these works, the authors have the freedom to vary packet transmission times and power levels which require sophisticated and expensive transmitter design. In the present work however, the controller does not have access to such rate control schemes. 
  %the authors assume knowledge of the channel state while transmitting as well as a rate control. 


The paper is organized as follows. We give our system model and the assumptions in
Section~\ref{sec:chanmodel}. We present the DP formulation of the problem
in Section~\ref{sec:dpalgo}.
We derive the theoretical bounds on the system performance in
Section~\ref{sec:bounds}. In Section~\ref{sec:simulation}, we analyze the
performance of the DP scheduler and compare it with the theoretical bounds. We
wrap up with a summary in
Section~\ref{sec:concl}.
%Once a practical packet scheduler is developed, we will derive the theoretical limits of the energy performance for 


==> simulation.tex <==
\section{Performance Evaluation}\label{sec:simulation}
\vspace{-0.1in}
%These simulations are performed for different scenarios by varying transition and loss probabilities of the 2SMC.
%technical report for this work~\cite{techrep}. 

%\subsection{Performance Metrics}
%Before presenting the simulation results, we introduce a few performance metrics that we will be using in this section. We define \emph{normalized transmission cost} as the 
%In this section we present the simulations based on the DP Algorithm developed in Section~\ref{sec:dpalgo} and compare it with the theoretical bounds. The power penalty incurred by the DP solution using ACK/NAK information is compared to the case when no channel estimation is done. These simulations are compared for a variety of channel conditions. Throughout these simulations, a two-state Markov channel is used. This choice is made due to the lower computational complexity of such a model, while retaining the insights that might be gained by a FSMC.

%Then we simulate the power penalty performance of the DP solution for ACK/NAK information with respect to the , and compare them for different channel conditions. A two-state Markov channel is used for the simulations
\subsection{Scheduler Performance and Theoretical Bounds}
\vspace{-0.1in}
We conduct simulations on FSMCs to compare the various transmission schedulers and compare them against their respective theoretical bounds.  
The metric used to compare the scheduler performance is termed \emph{normalized transmission cost} (NTC). We define $d$ as the number of data packets successfully transmitted in one time slot and NTC($d$) is the number of transmission attempts required to achieve this. For the theoretical bounds, the capacity-cost function $C(\mathcal{P})$, given by Theorem~\ref{th:capCSI} and Corollary~\ref{th:capACK}, is plotted as a function of the power constraint $\mathcal{P}$. Here $\mathcal{P}$ is equivalent to the number of packet transmission attempts made in a time slot. The capacity-cost function $C(\mathcal{P})$ is divided by the packet length $N$ to represent the capacity in terms of data packets and offer a direct comparison to the NTC.

%The transition probabilities for this model are given by $p_{21}=0.1$ and $p_{12}=0.2$. The loss probability in each state is $\epsilon_1=0.2$ and $\epsilon_2=0.8$. The time horizon $T$ for the simulations is 500 time slots and $10^5$ realizations of the channel are simulated. The packet error process is simulated by first generating a Markov process 500 time slots long and then setting the loss variable $z_k$ according to the given state $s_k$.
%The number of packets transmitted per unit time (averaged over all realizations) is plotted with respect to the normalized transmission cost. Normalized transmission cost is defined as the number of transmission attempts made per time slot to successfully transmit a particular quantity of packets. In this case, a packet is a data packet and the normalized transmission cost corresponding to $\delta$ packets is the number of attempts made in one time slot to successfully transmit $\delta$ packets. 

 %This normalized capacity is the number of packets that can be transmitted over the channel with an arbitrarily low probability of error. This is plotted for different power constraints, which can be thought of the number of packet transmission attempts made in a time slot.

%For the first set of simulations, we have selecte
\subsubsection{Comparison of DP-Schedulers for FSMCs}
Figures~\ref{fig:sim1} and~\ref{fig:3state} show the performance comparison of various DP-schedulers for 2- and 3-state Markov channels. The transition probabilities for the 2-state Markov channel (2SMC) are $p_{21}=0.1$ and $p_{12}=0.2$. The loss probability in each state is $\epsilon_1=0.2$ and $\epsilon_2=0.8$. For the 3-state Markov channel (3SMC), the transition probabilities are $p_{12}=0.025,\,p_{13}=0.075,\,p_{21}=0.075,\,p_{23}=0.05,\,p_{31}=0.05$ and $p_{32}=0.05$. The loss probabilities are $\epsilon_1=0.2,\,\epsilon_2=0.85$ and $\epsilon_3=0.95$. The time horizon $T$ for the simulations is 500 time slots and $10^5$ realizations of the channel are simulated. The packet error process is simulated by first generating a Markov process 500 time slots long and then setting the loss variable $z_k$ according to the given state $s_k$.

First, we plot the performance of DP-scheduler (solid red trace) and the corresponding bound (dashed red trace) for the non-causal perfect CSI case. For both cases (2SMC and 3SMC), the bound is tight up to the point when the deadline constraint requires a throughput of 0.2 packets/time slot. This can be due to the fact that for a lightly loaded system, the effect of queue state on decision making is minimal, and the scheduler considers CSI for decision making leading to a performance close to the theoretic bound. In all performance curves with feedback, for a 2SMC, a knee-point is observed when the NTC (or $\mathcal{P}$) is equal to 0.33 (for 3SMC, knee points at $\textrm{NTC}=0.37$ and $\textrm{NTC}=0.6$). As the number of packets to be transmitted is increased, the cost will increase at a certain rate since only the good states are being used initially. However after all the good states are exhausted, the scheduler will use the bad states for transmission, which increases cost at a faster rate as more packets will be dropped. For a throughput requirement of 0.25 packets/time slot in a 2SMC, causal perfect CSI scheduler requires 25\% more transmission attempts than a non-causal perfect CSI scheduler (10\% for a 3SMC). 

%The causal imperfect CSI based scheduler (black traces) shows a further drop in performance compared to the non-causal perfect CSI scheduler. 
We observe that the performance of the causal imperfect CSI scheduler or the ACK/NAK scheduler (solid black traces) is within 80\% of the theoretical bound (dashed black traces) for the 2SMC (75\% for the 3SMC). The bound is not very tight as the capacity calculations assume knowledge of the complete ACK/NAK sequence, whereas the ACK/NAK scheduler has access to the incomplete sequence (since ACK/NAK is unavailable for the time slots when no transmission is attempted). In both the cases, the ACK/NAK scheduler, at worst, requires 50\% more transmission attempts than the non-causal perfect CSI based scheduler for achieving a throughput of 0.25 packets/time slot.
%However, it is interesting to note that the ACK/NAK scheduler performs very close to the information theoretic bound (dashed black trace). In fact, the ACK/NAK-based scheduler achieves performance within 95\% of the theoretical bound. 
The green trace represents a blind transmission scheme.
In this case, the scheduler does not have any channel feedback, instead it just keeps transmitting till the queue is emptied out. This can be the lower bound on performance of any feedback scheme. The performance of this scheduler has a constant slope, since the scheduler does not adapt the transmission policy to the channel state. For a 2SMC, ACK/NAK scheduler outperforms the blind transmission scheme by up to 25\% for 0.1 packets/time slot throughput (50\% for a 3SMC) and 15\% for 0.25 packets/time slot throughput (20\% for a 3SMC). 
%As the energy constraint is increased to unity, all the controllers will attempt transmission in each slot regardless of the channel state. Hence, the performance of all the schemes will converge. 

%\subsubsection{Probe-based Scheduler}
%In Figure~\ref{fig:probe_comp}, we compare the performance of the ACK/NAK scheduler (dash-dot black trace) to the case when complete ACK/NAK information (solid blue trace) is available to the controller. 
%we consider a more realistic case, where ACK/NAK information is available only for time slots when a transmission is attempted (black dash-dot trace). The performance of this scheduler is compared to the case when the complete ACK/NAK sequence is available to the controller (blue solid trace).  
%To transmit 50 packets over 500 time slots, the ACK/NAK scheduler with complete ACK/NAK information requires 20\% fewer transmission attempts than the scheduler with incomplete ACK/NAK information. When the throughput requirement is increased to 125 packets over 500 time slots, this figure is reduced to 6\%. 
%On the other hand 
%This scheduler, delivers 20\% fewer packets for normal than the non-causal perfect CSI based scheduler.
%We observe that there is a substantial difference in performance of the scheduler when the complete and incomplete ACK/NAK information is available. However, we cannot assume such performance in practical systems as it is not reasonable to assume that complete ACK/NAK information will be available to the controller. 

%To bridge this gap between practicality and performance, we propose an probe-based scheduler. In this case, the controller has an option of sending either a full data packet or a probe packet (and incurring an associated cost). Since the probe packet does not carry any data, it has a transmission cost lower than that of a data packet. The underlying assumption being that the probe packet provides the same information about the wireless channel as a data packet (in terms of ACK/NAK). This assumption is not strictly valid since the error process for packets with different energies will be different. However, this idea of information provided by probe packets with different powers is beyond the scope of this work and it will be addressed in future work.

%In Figure~\ref{fig:probe_comp}, we use probe packets with cost = $\{0.05,0.1\}$ and plot their performance\footnote{Recall that the cost of a full data packet is 1.}. When the probe cost is equal to 0.05 (green dotted trace) the ACK/NAK scheduler requires a lower NTC for the same throughput requirement than the case when controller has incomplete ARQ information. At this cost, the channel should be probed to improve the performance of the ACK/NAK scheduler. On the other hand, when the probe cost is increased to 0.1 (blue dotted trace), the NTC of the probing scheduler for a given throughput becomes larger than the case when incomplete ARQ is available. Hence, for these channel parameters, when the probe cost is 0.1 the scheduler should use whatever information it has and not attempt to probe the channel. 
%\subsubsection{Comparison of DP-Schedulers for a 3-state Markov channel (3SMC)}
%In Figure~\ref{fig:3state}, we repeat the comparison for a 3SMC and observe similar trends. 
\subsubsection{Look-up Table Size}
Figure~\ref{fig:tablescaling} compares the effect of look-up table size on the performance of the ACK/NAK scheduler. The parameters for the 2SMC are: $p_{12}=0.18,\,p_{21}=0.09,\,\epsilon_1=0.23$ and $\epsilon_2=0.78$. The 32 MB table contains control action for $|\mathcal{A}|=256$ channel realizations and 20 levels of $\vec{w_k}$. The parameters for the 1 MB table are $|\mathcal{A}|=16$ and 10 levels of $\vec{w_k}$. Both tables store control action for upto 100 packets transmitted over a duration of upto 500 time slots. We observe that the ACK/NAK schedulers using a look-up table perform close to the exact solution. For instance, the 32 MB table requires 7\% extra transmission attempts (11.5\% for 1 MB table) to achieve throughput of 0.1 packets/time slot. Note that we have used uniform quantization for this example, however quantization methods that perform better might also exist.
\subsubsection{Time Horizon}
Figure~\ref{fig:time_horizon} compares the performance of the ACK/NAK scheduler with different time horizons $T$. The parameters for the 2SMC are: $p_{12}=0.2,\,p_{21}=0.1,\, \epsilon_1=0.1$ and $\epsilon_2=0.9$. We observe that with increasing $T$, the performance of the ACK/NAK scheduler improves. A scheduler with $T=100$ requires, at most, 10\% more transmission attempts than a scheduler with $T=800$.
%The maximum difference in performance for a ACK/NAK scheduler with $T=100$ and $T=800$ is 6\%. 
The improvement in performance can be due to the scheduler having greater flexibility in scheduling transmissions with larger $T$. We also observe that the performance of the ACK/NAK schedulers (for all $T$) is within 75\% of the theoretical bound.
\subsubsection{Terminal Cost}
In Figure~\ref{fig:terminal_cost}, we compare the effect of terminal cost $C$ on the performance of the ACK/NAK scheduler for a 2SMC. The channel parameters are: $p_{12}=0.2,\,p_{21}=0.1,\,\epsilon_1=0.2$ and $\epsilon_2=0.8$. For $C=\{10,50,200\}$, we observe that there is not much of a difference in the performance of the ACK/NAK schedulers formulated using these terminal costs. Other channel realizations also exhibit a similar behavior. This leads to the observation that the choice of $C$ does not impact the performance of the scheduler, as long as $C>10$.
\vspace{-0.2in}
\subsection{Power Penalty}
\vspace{-0.1in}
\subsubsection{Maximum Power Penalty}
We define the maximum power penalty for a feedback scheme using ACK/NAK information as $A_{\textrm{dB}}\triangleq \max_R 10\log_{10}\left(\frac{\text{Cost-Capacity for rate $R$ using ACK/NAK feedback}}{\text{Cost-Capacity for rate $R$ using causal CSI feedback}}\right)$. The Cost-Capacity function is the inverse of the Capacity-Cost function. Maximum power penalty quantifies the theoretical worst-case extra power required by an ACK/NAK based scheme to achieve the same throughput achieved by a causal perfect CSI based scheme. We define a similar quantity for the blind transmission scheme. 
Figure~\ref{fig:sim2th} compares the maximum power penalties incurred by ACK/NAK and blind schemes for 2SMCs as a function of channel memory $\mu\triangleq 1-p_{12}-p_{21}$. We plot this quantity for different values of loss probabilities $\{\epsilon_1,\epsilon_2\}$, while keeping the steady state probabilities $\{\pi(1),\pi(2)\}$ constant. The ACK/NAK based schemes do not incur a maximum power penalty of more than 1 dB. On the other hand, in case of no feedback (blind) the maximum power penalty can be as much as 4.5 dB. An interesting observation is that when the channel conditions are ``good'' ($\epsilon_1= 0.01$, $\epsilon_2= 0.1$) the advantage of using an ACK/NAK based scheme is negligible. In this case, the difference in $A_{\textrm{dB}}$ for the two cases is less than 0.1 dB. This can be explained by noting that under good channel conditions, there will be negligible packet drops and consequently, the value of estimating the channel is minimal.
\vspace{-0.05in}
\subsubsection{Actual Power Penalty}
Next, we find the actual power penalty incurred by an ACK/NAK scheduler, $L_{\textrm{dB}}\triangleq 10\log_{10}\left(\frac{\textrm{attempts made by ACK-NAK scheduler}}{\textrm{attempts made by causal CSI scheduler}}\right)$, for a given throughput. We define a similar quantity for the blind transmission scheme. 
Figure~\ref{fig:sim2} shows the power penalty incurred by the ACK/NAK based and blind schedulers for 2SMCs as a function of channel memory $\mu$. We plot this quantity for different values of packet loss probabilities, $\{\epsilon_1,\epsilon_2\}$ keeping the steady state probabilities $\{\pi(1),\pi(2)\}$ constant. 
%Power penalty $L_{\textrm{dB}}$ is defined as, $L_{\textrm{dB}}\triangleq 10\log_{10}\left(\frac{\textrm{attempts made by ACK-NAK/blind scheme}}{\textrm{attempts made by causal CSI scheme}}\right)$.
%In Figure~\ref{fig:sim2} for a particular packet loss probability model, the memory of the channel (defined as $1-g-b$) is varied and the power penalty, $L_{\textrm{dB}}\triangleq 10\log_{10}\left(\frac{\textrm{attempts made by ACK-NAK/blind scheme}}{\textrm{attempts made by causal CSI scheme}}\right)$.
For the range of channel parameters considered in our simulations and a throughput requirement of 0.2 packets/time slot, ACK/NAK scheduler does not incur a power penalty of more than 1.5 dB. On the other hand, a blind transmission scheme takes a power penalty of up to 4.5 dB (for $\epsilon_1=0$ and $\epsilon_2=1$).
%We also observe that as $(\epsilon_2-\epsilon_1)$ is decreased, the performance of all the schemes converge. This is explained by the fact that as $(\epsilon_2-\epsilon_1)\rightarrow 0$, the channel becomes i.i.d.~and any causal scheme to estimate the channel will fail since the channel state process is memoryless. %As a result, a scheduler that does not attempt to estimate the channel (e.g.,~blind scheduler) will be equivalent to a scheduler that does attempt to estimate the channel.

%\subsubsection{Varying Steady State Probabilities}
%We have performed additional simulations to find the power penalty, $L_{\textrm{dB}}$ incurred by an ACK/NAK based scheme and the blind transmission scheme. 
In Figure~\ref{fig:sim3}, 
%we plot the power penalty for the two transmission schedulers as a function of the channel memory $\mu$. Here, 
we consider different steady state probabilities $\{\pi(1),\pi(2)\}$, while keeping the loss probabilities constant ($\epsilon_1=0.1,\epsilon_2=0.9$). The throughput requirement is set at 0.1 packets/time slot.
%Figure~\ref{fig:sim3} shows the power penalty incurred by the ACK/NAK and blind transmission schemes as a function of channel memory, $\mu(=1-g-b)$ for different values of the steady state loss probabilities $\{\pi_\mathcal{G},\pi_\mathcal{B}\}$, while keeping the loss probabilities $\{p_g,p_b\}$ constant. 
%Power penalty $L_{\textrm{dB}}$ is defined as, $L_{\textrm{dB}}\triangleq 10\log_{10}\left(\frac{\textrm{attempts made by ACK-NAK/blind scheme}}{\textrm{attempts made by causal CSI scheme}}\right)$.
%In Figure~\ref{fig:sim2} for a particular packet loss probability model, the memory of the channel (defined as $1-g-b$) is varied and the power penalty, $L_{\textrm{dB}}\triangleq 10\log_{10}\left(\frac{\textrm{attempts made by ACK-NAK/blind scheme}}{\textrm{attempts made by causal CSI scheme}}\right)$.
In the worst case, the ACK/NAK scheduler incurs a power penalty of 2.5~dB for $\pi_1=0.2$ and $\pi_2=0.8$ whereas the blind scheme incurs a power penalty of almost 4.5~dB. For $\mu=0.9$, in all the cases, the performance of the ACK/NAK scheduler is 2 dB better than the blind scheduler. 
%This is due to the fact that for a two-state Markov channel with these parameters, ACK/NAK is equivalent to the causal CSI. In this case, the blind transmission scheme takes a power penalty of upto 4.5 dB (solid blue trace).
%We note that since we have chosen values of loss probability $\{p_\mathcal{G},p_\mathcal{B}\}$ that show a significant difference in performance of the blind and ACK/NAK based schemes. As we have observed in Figure~\ref{fig:sim2}, the performance of all the schemes converge when the difference between the loss probabilities is reduced, as a result, we do not expect considerable improvements in performance in such cases. 
Since $\mu$ is an indicator of the burstiness (as bursty channels have high values of $\mu$), the improvement provided by our scheme will be more pronounced in bursty channels.


%The proportional change is always negative for the blind scheme indicating that, for the range of values considered for our simulations, a scheduling algorithm based on an ACK/NAK scheme will perform better in terms of energy efficiency than a blind scheme. On the other hand, a scheme that uses causal CSI always performs better than a ACK/NAK based scheme. When the channel memory ($1-g-b$) is high then the performance of an ACK/NAK based scheme is substantially better than a blind scheme, however the ``cost'' using ACK/NAK information instead of causal CSI is not significant. When $p_g=0$ and $p_b=1$, then the ACK/NAK based scheme and causal CSI scheme are the same, as the ACK/NAK is equal to the CSI. As a result, we do not see any difference in performance between the two scheme. As the difference between the loss probabilities ($p_b-p_g$) decreases the performance of all the schemes become similar. This is also expected, as when $p_b=p_g$, we have an independent and identically distributed (i.i.d.) loss model. For an i.i.d. model, the previous state information is not of any use, as a result all the three schemes will perform identically.

%On the other hand, the performance of blind transmission scheme is substantially lower than the  However, the difference in performance for a causal CSI based scheme vis-\`a-vis
%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{performance_improv_ssprob.eps}
%\caption{The proportional change in performance with respect to change in channel memory for different values of steady state probabilities $\{\pi_g,\pi_b\}$. The throughput is kept constant at 0.2 packets/time slot for all cases and $p_g=0.2$ and $p_b=0.8$.} \label{fig:sim3}
%\end{figure}
%We plot the same quantities, but this time for different steady state probabilities $\{\pi(\mathcal{G}),\pi(\mathcal{B})\}$ and keeping the packet loss probabilities constant. We observe that the ACK/NAK based scheme outperforms the blind transmission scheme. In fact, for some cases it requires only half the number of transmission attempt to achieve the same throughput. On the other hand, the drop in power consumption performance due to the lack of causal CSI is not substantial. 


